New Renormalization Group Results for Scaling of Self-Avoiding Tethered Membranes

The scaling properties of self-avoiding polymerized 2-dimensional membranes are studied via renormalization group methods based on a multilocal operator product expansion. The renormalization group functions are calculated to second order. This yields the scaling exponent nu to order epsilon^2. Our extrapolations for nu agree with the Gaussian variational estimate for large space dimension d and are close to the Flory estimate for d=3. The interplay between self-avoidance and rigidity at small d is briefly discussed.

==> f-nuLd+2R-D-eps.tex <==
%auto-ignore
\begin{figure}[htb] 
\centerline{
\Dd{1}{2}%
\epsfxsize=8.0cm \parbox{8.0cm}{\epsfbox{./eps/nudp2_D_eps_1_2.eps}}
\hspace{0.0cm}
\Dd{1}{3}%
\epsfxsize=8.0cm \parbox{8.0cm}{\epsfbox{./eps/nudp2_D_eps_1_3.eps}}
}
\centerline{
\Dd{2}{2}%
\epsfxsize=8.0cm \parbox{8.0cm}{\epsfbox{./eps/nudp2_D_eps_2_2.eps}}
\hspace{0.0cm}
\Dd{2}{3}%
\epsfxsize=8.0cm \parbox{8.0cm}{\epsfbox{./eps/nudp2_D_eps_2_3.eps}}
}
\centerline{
\Dd{2}{6}%
\epsfxsize=8.0cm \parbox{8.0cm}{\epsfbox{./eps/nudp2_D_eps_2_6.eps}}
\hspace{0.0cm}
\Dd{2}{20}%
\epsfxsize=8.0cm \parbox{8.0cm}{\epsfbox{./eps/nudp2_D_eps_2_20.eps}}
}
\caption{Extrapolation of $\nu(d+2)$ in $D$ and $\E$ to $(D,d)=$ (1,2), (1,3), (2,2),
(2,3), (2,6), (2,20). Eventhough this extrapolation semms to converge best, it is 
bad, as the result for membranes is completely independant of $d$. One should take
this as a warning with respect to beautifully looking curves!}
\label{f: nu(d+2)-D-eps}
\end{figure} 


==> f-nudtab.tex <==
%auto-ignore
\begin{figure}[tb]\centerline{ \renewcommand{\arraystretch}{1.2}
\begin{tabular}[t]{|l|c|c|c|c|c|c|} \hline
$(D,d)$ & $(1,1)$ & $(1,2)$ & $(1,3)$ & $(2,2)$ & $(2,3)$ & $(2,20)$
\\ \hline \hline 
$d\nu_{\mbox{\scriptsize exact}}$ & 1 & 1.5 & $ 1.758 \pm 0.012$ & 2  & ???  & ???
\\ \hline
$d\nu_{\mbox{\scriptsize Flory}}$ & 1 & 1.5 & 1.8 & 2 & 2.4 & 3.636
\\ \hline
$d\nu_{\mbox{\scriptsize var}}$ & 2 & 2 & 2 & 4 & 4 & 4
\\ \hline
$d\nu_{D,\,D_c(d)}^{\mbox{\scriptsize left cut}}$ & 1.09 & 1.39 & 1.74 & 1.94 &
2.37 & 3.95
\\ \hline
$d\nu_{D,\,D_c(d)}^{\mbox{\scriptsize right cut}}$ & 2.08 & 1.52 & 1.81 & 2.09 & 2.47 & 4.10
\\ \hline
$d\nu_{D,\,D_c(d)}^{\mbox{\scriptsize mid cut}}$ & 1.59 & 1.46 & 1.78 & 2.02 & 2.42 & 4.03
\\ \hline
\end{tabular}  \renewcommand{\arraystretch}{1.0} }
\caption{Results of the numerical extrapolations for $\nu d$.
If not stated otherwise  the error is $\pm 1$ in the last digit.}
\label{nudtab}
\end{figure}%

